Expanding the Design Space for Electrically-Driven Soft Robots through Handed Shearing Auxetics

Handed Shearing Auxetics (HSA) are a promising structure for making electrically driven robots with distributed compliance that convert a motors rotation and torque into extension and force. We overcame past limitations on the range of actuation, blocked force, and stiffness by focusing on two key design parameters: the point of an HSA's auxetic trajectory that is energetically preferred, and the number of cells along the HSAs length. Modeling the HSA as a programmable spring, we characterize the effect of both on blocked force, minimum energy length, spring constant, angle range and holding torque. We also examined the effect viscoelasticity has on actuation forces over time. By varying the auxetic trajectory point, we were able to make actuators that can push, pull, or do both. We expanded the range of forces possible from 5N to 150N, and the range of stiffness from 2 N/mm to 89 N/mm. For a fixed point on the auxetic trajectory, we found decreasing length can improve force output, at the expense of needing higher torques, and having a shorter throw. We also found that the viscoelastic effects can limit the amount of force a 3D printed HSA can apply over time.

==> futurework.tex <==



==> scrap.tex <==
%largely finalized                                            
Starting at -180 degrees, as the angle of twist increases so does the blocked force according to Fig. 5a. The blocked force trends are largely what we expected.  Blocked force is the force exerted on the load cell by an HSA at its printed rest length for any arbitrary rotation value. This is important because as the HSA is rotated, the position of the minimum energy state changes. The difference in position between the printed rest length and the minimum energy state induces a spring potential energy on the HSA; the further apart these two positions are, the stronger the pull is toward the minimum energy state. This explains why higher angles of twist have a higher magnitude of blocked force: the distance between the minimum energy state and printed length is higher, which coincides with a higher spring potential energy. For example, at -180 degrees is the lowest in this range at -3.4 mm below the print length. When blocked force is obtained at the print length, the HSA wants to close 3.4 mm because of the aforementioned potential energy. The top of the HSA is fixed in place by the load frame, which means the HSA will naturally try to pull on the lower clamp of the load frame which induces a pulling (negative) force on the cell.  

%word vomit to be adjusted
that being said, why the cubic behavior of the semi open HSA? why does it not decrease or increase in blocked force to the same extent that the other configurations do? why does it seem like there are clearer limits to the blocked force its capable of, or why it dies out so quickly? \tosh{WAIT TO WRITE UNTIL WE MEET WITH ADITYA AND JEFF TO TALK ABOUT EDGE OF CYCLE ERROR} I have come to think its because of the high ratio of minimum energy displacement to extension range seen only in the semi-open configuration... well, that's true for the fully open HSA as well so why does the same cubic behavior not arise? Is it because the rest length, where blocked force is recorded, is always above the minimum energy state so the curve doesnt have any inflection points?


It is observed that the rate of increase of the magnitude of the blocked force versus the angle of rotation for the fully open HSA is significantly greater than the closed and the semi-open HSAs. This is because the initially vertical primary bands are hard to deform, hence a twist applied to a fully open HSA results in significantly more energy being stored compared to the same amount of twist for other two HSAs.

As for holding torque, the data makes sense. The resting state, in terms of torque, for all HSAs is at 0 degrees rotation. The more you rotate away from this point, the more potential energy you have for twisting back to that resting state. We need an explanation for the cubic nature of the semi-open. Edge error? Printing error? Need to discuss

\tosh{Also wait to write about spring constant and holding torque for semi open until we meet with jeff and aditya and update the plots}

The general trend on Fig 5b suggests that spring constant increases in magnitude drastically as the angle of twist is reduced. However, when the angle of twist is reduced the geometry should be less suited to carrying a transverse load. (why? reduction in cross sectional area? polar moment of inertia?) If that's the case, why does the data look like this? The answer lies in our testing procedure, namely the cycling range; the open HSA was tested entirely in compression. If we would have tried to extend the open HSA beyond its rest length at any point, the spring constant trend would have been what was originally expected. Data was collected on the upcycle, which is where the HSA moves from minimum to maximum. The lower cycling limit for the open HSA is defined as the minimum energy state at -180 degree rotation. If data is taken on the upcycle, that is, moving away from this minimum energy state back toward the rest length, it makes sense that as angle of twist increases (and therefore the minimum energy state moves closer to the printed rest length) it takes less energy to move the HSA on the upcycle. This is analogous to the spring constant getting smaller in magnitude. In the case of the closed 4 row HSA that's tested entirely in tension with a cycling range of 0 mm to 20 mm, the spring constant generally increases as a function of angle of twist; this is what we originally expected. As the HSA opens up, the geometry becomes better suited to resisting extension. While the minimum energy state does move up, the ratio of that increase to the overall extension range is small which is why we see a general increase to spring constant on the closed HSA. On the semi-open HSA on the other hand, the ratio of minimum energy state displacement to its extension range is much larger. This explains why the spring constant seems to drop as the angle of twist rises: above zero degrees angle of twist, the position of the minimum energy state rises to XXX. The upper limit of the displacement range is XXX, so it's actually favorable for the HSA to be extended toward the top during its upcycle. THe degree to which this is favorable depends entirely on the ratio of minimum energy displacement to the limits of displacement when cycling. 

The closed HSA requires a greater counterclockwise torque as the counterclockwise rotation applied at its end is increased and the fully open HSA requires a greater clockwise torque as the clockwise rotation applied at its end is increased. The semi-open HSA requires a greater clockwise torque as the clockwise rotation applied at its end is increased and a greater counterclockwise torque as the counterclockwise rotation applied at its end is increased. The holding torque for the semi open for a 90 degree counterclockwise rotation drops for the same reason as the blocked force. 
The rate of increase of the magnitude of the holding torque versus the angle of rotation for the closed HSA is significantly greater than the semi-open and the fully open HSAs. This could be because as the primary bands get close to being vertical, they resist less torque and less material deforms and hence resulting in less energy required to go from one rotation state to the other.
\tosh{ \printinunitsof{in}\prntlen{\linewidth} (linewidth for reference). minimum energy length. ACKNOWLEDGED, MAKING TABLE}


% \begin{itemize} 
%     \item  \aditya{Block force}
    The blocked force required as a function of the angle of rotations for the HSAs with varying row counts is shown in Fig. 6(a). The blocked force is 0N when no rotation is applied. All the HSAs require a greater pulling force as the angle of rotation is increased. We observed that the rate of increase of the blocked force is inversely proportional to the number of rows squared. There is a spike in the blocked force for the 12 row HSA after a rotation of 150 degrees because the HSA begins to buckle.
%        \item \aditya{Spring Constant}
    The spring constant as a function of the angle of rotations for the HSAs with varying row counts is shown in Fig. 6(b). The spring constant for the HSAs stays relatively constant as the rotation is increased except for the 4 row and 6 row HSAs. This is also seen in Table II where the slopes of the linear fits to the spring constant data are closely matched except for the 4 row and 6 row HSAs. The spring constant continuously increases for the 4 row HSA and for the 6 row HSA after 60 degrees because at that amount of twist, the primary and secondary bands are so far apart that the bulk material of the HSA beings to deform instead of the auxetic unit cells changing shape.
%        \item \aditya{holding torque @min energy length}
    The holding torque as a function of the angle of rotations for the HSAs with varying row counts is shown in Fig. 6(d). The holding torque is 0Nmm when no rotation is applied. All the HSAs require a greater holding torque as the angle of rotation is increased. The rate of increase of holding torque is inversely proportional to the number of rows; shown in Table II by the decreasing slope of the linear fit to the holding torque data as the number of rows increases. This is because the deformation per unit length is greater for a smaller HSA.
%\end{itemize}        


These trends are what we expected. Shorter HSAs are much better at carrying large amounts of torque. More rows = more free space for hysteresis and creep to cause torque to fizzle out (describe this smarter). On shorter HSAs, the lower amount of empty space in the middle carries an intrinsic resistance to adverse side affects such as creep and hysteresis due to their lower density of stress concentrators; stress doesn't have to 'travel' far in shorter HSAs. In longer HSAs
